Open-Source Internships With Industry Mentors

Internships help students connect what they have learned in the classroom to the real world, and students with access to internships are more likely to graduate and secure employment. However, many students are unable to find an internship by the time they graduate. This experience report describes a program where volunteer software engineers mentor students as they work on open-source projects in the summer, offered as an alternative to a traditional internship experience. We catalog the considerations involved in providing an experience similar to a traditional internship, describe our program's design, and provide two years' worth of participant evaluations and career outcomes as a measure of efficacy. The program served mostly undergraduates from non-R1 schools who are underrepresented in technology, and achieved similar educational outcomes to a traditional internship program. Most promisingly, mentors were willing to serve as a professional reference for 80% of students and the number of graduating seniors who secured full-time employment in technology was 7 points higher than average (despite occurring during the COVID-19 pandemic).

==> meta/conf.tex <==
\setcopyright{acmcopyright}
\copyrightyear{2022}
\acmYear{2022}


\copyrightyear{2022}
\acmYear{2022}
\setcopyright{acmlicensed}
\acmConference[ITiCSE 2022] {Proceedings of the 27th ACM Conference on Innovation and Technology in Computer Science Education Vol 1}{July 8--13, 2022}{Dublin, Ireland.}
\acmBooktitle{Proceedings of the 27th ACM Conference on Innovation and Technology in Computer Science Education Vol 1 (ITiCSE 2022), July 8--13, 2022, Dublin, Ireland}
\acmPrice{15.00}
\acmDOI{10.1145/3502718.3524763}
\acmISBN{978-1-4503-9201-3/22/07}
% Authors, replace the red X's with your assigned DOI string during the rightsreview eform process.

